Concolic Testing for Deep Neural Networks

Concolic testing combines program execution and symbolic analysis to explore the execution paths of a software program. This paper presents the first concolic testing approach for Deep Neural Networks (DNNs). More specifically, we formalise coverage criteria for DNNs that have been studied in the literature, and then develop a coherent method for performing concolic testing to increase test coverage. Our experimental results show the effectiveness of the concolic testing approach in both achieving high coverage and finding adversarial examples.

==> LipschitzTest.tex <==
\subsection{Algorithms for Lipschitz Test Case Generation}

%\wenjie{This section is reserved for wenjie writing lipschitz test case generation, will delete this mark once finished}

Given a network $f$, a legimate input $x_0 \in \mathbb{R}^n$ and a predefined Lipschitz constant $c$, we need to generate two inputs or a test pair $x_1$ and $x_2$ such that 
\begin{equation}
\begin{split}
\dfrac{|| f(x_1) - f(x_2)||_{D_1}}{||x_1 - x_2||_{D_1}} > c \\
\text{s.t.~~} || x_1 - x_0 ||_{D_2} \leq \Delta \\
                    || x_2 - x_0 ||_{D_2} \leq \Delta 
\end{split}
\end{equation}
where $f(x)$ represents the chosen logit or probabilistic confidence output of a network, $||*||_{D_1}$ and $||*||_{D_2}$ denote certain norm metric such as $L_0$-norm, $L_2$-norm or $L_{\infty}$-norm, and $\Delta$ intuitively represents the radius of a norm ball (for $L_1, L_2$-norm) or size of a hypercube (for $L_{\infty}$-norm) centered on $x_0$.

We formulate the above satisfication problem as an optimisation problem which can be efficiently solved by an {\em alternative compass search} scheme. Specifically, we alternatively optimise the following two optimisation problems.
%
\subsubsection{Stage One} we solve
	\begin{equation}\label{eqn-27}
	\begin{split}
	\min_{x_1} \mathbf{Lip}(x_1,x_0) = - \dfrac{|| f(x_1) - f(x_0)||_{D_1}}{||x_1 - x_0||_{D_1} + \epsilon} \\
	\text{s.t.~~} || x_1 - x_0 ||_{D_2} \leq \Delta
	\end{split}
	\end{equation}
	where $\epsilon$ is a very small positive constant to avoid the case that denominator equals to zero. Obviously $\mathbf{Lip}(x_1,x_0)$ is the negative of Lipschitz constant of $x_1$ and $x_0$. The above objective enables the algorthm to search an optimal $x_1$ in the space of a norm ball or hypercube centered on $x_0$ with radius $\Delta$, such that the Lipschitz constant of $x_1$ and $x_0$ as large as possible. 
	 
	To solve the above the problem, we use the compass search method which is efficient and derivetive-free, and most importantly, guarantteed to have first-order global convergence~\cite{audet2017derivative}. Because we aim to find a test pair to break the predefined Lipschitz constant $c$ instead of finding the largest Lipschitz constant. As a result, along each iteration when we get $\bar{x}_1$, we do a satisfication checking by evaluating whether $ -\mathbf{Lip}(\bar{x}_1,x_0) > c$ holds. If it holds, we then find an image pair $\bar{x}_1$ and $x_0$ satisfies the test requirement; if it does not hold, we continue the compass search until the final convergence  or satisfied image pair generated. If the Eqn.~\ref{eqn-27} is convergent and we can find an optimal $x_1$ as
	$$
	x_1^* = \arg\min_{x_1}\dfrac{|| f(x_1) - f(x_0)||_{D_1}}{||x_1 - x_0||_{D_1} + \epsilon}
	$$
	but we still cannot find an satisfied image pair, we do the step-2 optimisation.
	
	\subsubsection{Stage Two} we solve 
	\begin{equation}\label{eqn-28}
	\begin{split}
	\min_{x_2} \mathbf{Lip}(x_1^*,x_2) = \dfrac{|| f(x_2) - f(x_1^*)||_{D_1}}{||x_2 - x_1^*||_{D_1}+\epsilon} \\
	\text{s.t.~~} || x_2 - x_0 ||_{D_2} \leq \Delta
	\end{split}
	\end{equation}
	Similarly, we use derivetive-free compass search to solve the above problem and checking whether $ -\mathbf{Lip}(x_1^*,x_2)> c$ holds at each iterative optimisation trace $\bar{x}_2$. If it holds, we then return the image pair $x_1^*$ and $\bar{x}_2$ satisfies the test requirement; if not hold, we continue the optimisation until the final convergence or satisfied image pair generated. If Eqn.~\ref{eqn-28} is convergent at $x_2^*$, we still cannot find such test pair, we again modifiy the objective function by enabling $x_1^* = x_2^*$ in Eqn.~\ref{eqn-28}  and continue such searching and satisfication checking procedure.
	
	\subsubsection{Stage Three: } When on Stage Two, no matter how we alternatively change the objective function, the objective function $\mathbf{Lip}(x_1^*,x_2^*)$ stops decreasing. We then treat the whole searching procedure convergent and fail to find such an image pair that can break the predefined Lipschitz Constant $c$. In this case, we will return the best image pair we can find, i.e., $x_1^*$ and $x_2^*$, and the largest Lipschitz constant we can find $-\mathbf{Lip}(x_1^*,x_2)$ although it is smaller than $c$.
	
	In summary, the proposed method is an alternative optimisation scheme based on the compass search. Bascially, we start from the given $x_0$ to search an image $x_1$ in a norm ball or hypercube (the optimisation trajectory on the norm ball space is denoted as $S(x_0,\Delta(x_0))$) such that $Lip(x_0,x_1)>c$ (this step is symbolic excution), if cannot find, we modify the optimisation objective function by replacing $x_0$ with $x_1^*$ (the best concrete image find in this optmization trace) to initiate another optimisation trajectory on the space, i.e., $S(x_1^*,\Delta(x_0))$, so on so forth, our optimisation trace can gradually cover the whole norm ball space $S(\Delta(x_0))$.





==> app_LipConstTest.tex <==
\subsection{Settings for Lispchitz Constant Coverage}
\label{app:LipConstTest}

\subsubsection{Model Structures of MNIST DNN}

See Table \ref{tab:lisp-mnist}.

\begin{table}
	\vspace{5mm}
	\caption{MNIST DNN for Lipschitz Coverage}
	\label{tab:lisp-mnist}
		\vspace{3mm}
\centering
	\begin{tabular}{ l | c }
		\toprule
		Layer Type & Size\\
		\hline
		Input layer & 28 $\times$ 28 $\times$ 1 \\ 
		Convolution layer & 3 $\times$ 3 $\times$ 16  \\ 
		ReLU activation & \\
		Convolution layer & 3 $\times$ 3 $\times$ 32  \\
		Batch-Normalization layer & \\
		ReLU activation & \\
		Convolution layer & 3 $\times$ 3 $\times$ 64  \\
		Batch-Normalization layer & \\
		ReLU activation & \\
		Convolution layer & 3 $\times$ 3 $\times$ 128  \\
		Batch-Normalization layer & \\
		ReLU activation & \\
		Dropout layer & 0.5 \\
		Fully Connected layer & 256  \\ 
		ReLU activation & \\
		Dropout layer & 0.5 \\
		Fully Connected layer & 10  \\ 
		Softmax + Class output &   \\ 
		\bottomrule    
	\end{tabular}
		\vspace{5mm}
\end{table}



\subsubsection{Model Structures of CIFAR-10 DNN}

See Table \ref{tab:lisp-cifar}

\begin{table}
	\vspace{5mm}
	\caption{CIFAR-10 DNN for Lipschitz Coverage}
	\label{tab:lisp-cifar}
	\vspace{3mm}
	\centering
	\begin{tabular}{ l | c }
		\toprule
		Layer Type & Size\\
		\hline
		Input layer & 32 $\times$ 32 $\times$ 3 \\ 
		Convolution layer & 3 $\times$ 3 $\times$ 32  \\ 
		ReLU activation & \\
		Convolution layer & 3 $\times$ 3 $\times$ 32  \\ 
		ReLU activation & \\
		Maxpooling layer & 2 $\times$ 2\\
		Dropout layer & 0.5\\
		Convolution layer & 3 $\times$ 3 $\times$ 64  \\ 
		ReLU activation & \\
		Convolution layer & 3 $\times$ 3 $\times$ 64  \\ 
		ReLU activation & \\
		Maxpooling layer & 2 $\times$ 2\\
		Dropout layer & 0.5\\
		Fully Connected layer & 512  \\
		ReLU activation & \\
		Fully Connected layer & 10  \\ 
		Softmax + Class output &   \\ 
		\bottomrule    
	\end{tabular}
		\vspace{5mm}
\end{table}


\subsubsection{DNN Training Setup} 

\begin{itemize}
	\item Hardware: Notebook PC with I7-7700HQ, 16\,GB RAM, GTX 1050 GPU
	
	\item Software: Matlab 2018a, Neural Network Toolbox, Image Processing Toolbox, Parallel Computing Toolbox, Optimization Toolbox
	
	\item Parameter optimization settings: SGDM, Max Epochs = 30, Mini-Batch Size = 128
	
	\item Training dataset: MNIST training dataset with 50,000 images; CIFAR-10 training dataset with 50,000 images
	
	\item Training accuracy: 100\% for MNIST; 95.3\% for CIFAR-10.
	
	\item Testing dataset: MNIST testing dataset with 10,000 images and CIFAR-10 testing dataset with 10,000 images
	
	\item Testing accuracy: 99.46\% for MNIST and 76.6\% for CIFAR-10
\end{itemize}


\subsubsection{Algorithm Setup} 
\begin{itemize}
	\item $\Delta = 0.1$
	
	\item The maximum number of iterations on each compass search is $150$
	
	\item The maximum number of concolic executions is $30$ for an input image
	
	\item Tested Images: Image-1 to Image-50 from the testing datasets of MNIST and CIFAR-10 
\end{itemize}


==> response.tex <==
\newpage
\section*{Responses to the Reviewers}

We thank the reviewers for their insights. This letter summarises our revision regarding
the metareview and individual reviews.

\subsection*{Metareview}

\begin{revPoint}
Coherent use of the QLAR logic across the paper (or removal of the QLAR logic, if deemed inadequate based on the reviewers' comments)
\begin{quote}
Thank you for pointing this out. We made a major revision to the logic to make sure that all the inconsistencies are amended. The detailed revision information is as follows. 

In the last submission, we used this logic to express both  testing requirements and their corresponding optimisation expressions. Optimisation expressions are used later in requirement evaluation and symbolic generation of new concrete inputs. An inconsistency appears because requirements are Boolean and optimisation expressions return inputs. In the new version, we separate the testing requirements and their optimisaiton expressions. In Section 4, the logic QLAR is used solely for the expression of testing requirements, and therefore optimisation operators are excluded from QLAR. The optimsiaiton expressions are introduced later when needed, i.e., for requirement evaluation in Section 7. % and for symbolic test case generation in Section 8. 

Another inconsistency mentioned is on the nested usage of requirement $r$ and Boolean formula $e$. By the logic syntax, $e$ can be a subformula of $r$, but not vice versa. That is, we do not allow the quantifiers $Q$ to appear in a formula  more than once. All the example requirements in the paper follow this restriction. In the  submission, there was an oversight in a statement mentioning that a variable cannot be quantified by multiple quantifiers. This statement has been removed in the new version as such cases are not allowed by the logic syntax.  
%We simplified QLAR syntax (Section \ref{sec:qlpr}) and clarified the semantic for "the
%satisfiability of a requirement $r$ over a test suite $\testsuites$" (Section \ref{sec:semantics}).
\end{quote}

\end{revPoint}


\begin{revPoint}
Better (self-contained) description of the LP problem.
\begin{quote}
A detailed explanation of the LP modeling problem is now added (Section 8.1).

The Linear Programming (LP) model (denoted as $\mathcal{C}$ for generic purpose)
by \eqref{eq:lp-v} and \eqref{eq:lp-dir1} encodes a particular activation pattern.
The linear constraints in \eqref{eq:lp-v} denote a symbolic version of the computation of 
a neuron's activation defined in \eqref{eq:sum}. Similarly, the set of linear constraints in
\eqref{eq:lp-dir1} encode every neuron's ReLU operation \eqref{eq:relu}. Though ReLU is a non-linear operation,
when the activation pattern is fixed, it is either activated or de-activated.

The linear model $\mathcal{C}$ represents an input set that
produce  the same activation pattern as encoded. "Consequently,
the symbolic analysis for finding a new input $t'$ from a pair $(t, r)$ of 
input and requirement is equivalent to finding a new activation pattern. Note that,
to make sure that the obtained test case is meaningful, in the LP model an objective
is added to minimize the distance between $t$ and $t'$. Thus, the use of LP requires that a distance metric
be linear, e.g., $L_{\infty}$-norm." The linear encoding of the Chebyshev distance $L_{\infty}$ is as in
\eqref{eq:chebyshev}.


Given the test case $t$ and requirement $r$
that is chosen by the heuristic, a new activation pattern is created to satisfy the requirement $r$
(Section 8.1.1, 8.1.2 and 8.1.3). This pattern is encoded by the LP modeling as \eqref{eq:lp-v} and 
\eqref{eq:lp-dir1} and its solution (if it is feasible) will be the new concrete input (that satisfies $r$).


As we put in the end of Section 8.1.1 
"Finally, the new activation pattern defined in \eqref{eq:lp-nc} is encoded by the LP model $\mathcal{C}$
as \eqref{eq:lp-v} and \eqref{eq:lp-dir1},
and if there exists a feasible solution, then it will become the new test case $t'$, which makes the DNN
satisfy the requirement $r$"
\end{quote}

\end{revPoint}

\begin{revPoint}
Further explanations on the experimental part, as requested in the reviews.
\begin{quote}
More details are added into the experiment as indicated by reviewers. 

\begin{itemize}
    \item The implementation and all data in the experiment are now available online at 
    \url{https://github.com/TrustAI/DeepConcolic}.
    \item We specify a threshold of 12 hours for each DeepConcolic run.
    When testing a DNN, if the DeepConcolic testing does not finish within 12 hours, it is forced to terminate.
    \item All coverage results are collected by running the testing repeatedly at least 10 times.
    The full coverage report, including the average coverage and standard derivation, is
    given in Figure~\ref{fig:coverage}. 
    The experiment results in Table \ref{tab:NC+DeepConcolic+DeepXplore} and \ref{tab:cover-results} have been
    also updated. 
    \item For the scalability of our approach, we note that, among the three symbolic algorithms (linear programming, global optimisation, and Lipschitz test generation), the last two have been shown to be scalable to large, state-of-the-art networks including imageNet networks such as ResNet, VGG-16, VGG-19 etc. See [21] for some preliminary results for the global optimisation approach on large networks. For the linear programming, due to technical reason (encoding of hidden layers), we haven't been able to conduct experiments on large networks. But given the fact that linear programming is in polynomial time, we believe it is possible. Please refer to the detailed response to the reviewers' questions below for more information. 
    %Unfortunately, the current DeepConcolic implementation does not support other DNN models used in DeepXplore.
    %The problem here is that DeepConcolic now only recognises DNN models that are trained following our customised 
    %architecture and the training of models like VGG16 really requires some dedicated efforts. [xiaowei: not happy with this answer. what do you mean by customised architecture? ]
    %We haven't extend DeepConcolic to work with other models
    %\item The DNN models used in the paper are medium-sized that can be already of interest for some industrial applications.
    %The usage of DeepConcolic on even bigger DNN models will depend on the scalability of the Linear Programming (LP) problem.
 \end{itemize}
\end{quote}

\end{revPoint}

\subsection*{Review \#519A}

\begin{revPoint}
It is concolic in the following sense: it starts from concrete input images and attempts to find similar ones.
However, this is not as new as is being claimed: several other approaches can start from a concrete image and attempt to apply linear programming or SMT solving: 

[15] "Safety verification of deep neural networks"

[16] "Reluplex: An efficient SMT solver for verifying deep neural networks"
     
     "Reachability analysis of deep neural networks with provable guarantees": https://arxiv.org/abs/1805.02242

and similar results using stochastic search: "Feature-guided black-box safety testing of deep neural networks"

\begin{quote}

Thank you for mentioning these related works. Among the four papers mentioned, three of them are authored by our group. So we have a full understanding of these works. The approach proposed in this paper is significantly different. % with them.
We have discussed this in the related work, but would like to provide more details here. 

All the mentioned papers are verification methods, aiming to prove or disprove safety of a network. On the other hand, the concolic approach in this paper aims  to provide coverage of the test requirements, instead of the formal guarantees on the safety property.

There are also differences  in the detailed methods: [15] discretizes the vector space of each hidden layer and conducts a layer-by-layer analysis, [16] encodes the  neural network into 
an SMT model, the IJCAI paper on reachability analysis develops a global optimisation approach to compute the safety radius, and the TACAS paper on feature-guided black-box testing reduces the safety verification to a two-player game to enable its solution by Monte Carlo tree search. All of them can be seen as either concrete execution or symbolic execution, but not their interleaving/combination (i.e., concolic). On the other hand,  the concolic testing in this paper considers both concrete execution and symbolic execution. Moreover, for symbolic execution,
approaches based on linear programming  (for test metrics) and local optimisation  (for Lipschitz requirements) are employed. 

%given a concrete input, we only encode the linear constraints around it, which reserve
%the same linear behavior/activation pattern (Definition \ref{def:activation-pattern}) of the neural network.

%"Feature-guided black-box safety testing of deep neural networks" features blackbox testing with Monte Carlo Tree Search, whereas ours is a whitebox testing technique.
\end{quote}

\end{revPoint}


\begin{revPoint}
As to the concolic part: determining *which* concrete image to select is not really discussed; from the description in Section 7 it is unclear whether every concrete image is tried, in which case, it is really just trying out symbolic methods against all images and so little different than trying the above references systematically against all inputs.  The interplay between random generation and systematic exploration (in normal concolic testing) is quite different than what is proposed here.
\begin{quote}
Our concolic method does not apply symbolic execution on every concrete input. Instead, we maintain a set of test cases (concrete inputs), evaluate them against the test requirements with respect to heuristic functions, select the most promising pair (test case, test requirement), apply  symbolic execution to find a next test case, and then add the new test case into the maintained set. 

In other words, to see if we can find a test case to satisfy a given test requirement, we start from a random input, conduct concrete execution until it gets stuck, and then apply symbolic execution to find a next test case. This procedure largely follows the usual concolic testing. 

%Our method does not try all inputs, and that is something we try to avoid. Our algorithm is directed by the set of pre-defined properties (due to the test criterion used) and it explores the input space so as to satisfy the set of properties as much as possible.
\end{quote}

\end{revPoint}


\begin{revPoint}
The QLAR logic, as described in Section 4A, is not well-typed.  Some top-level queries return a Boolean value (quantified formulas), and some return a real value (for the opt formulas), so the objects in "r" are of ambiguous type.  Also, I am confused by the syntax vs. semantic definitions: since "r" never appears on the right side of the grammar, I do not see how some of the constructions in the semantics (Section 4.B) can be created.  Perhaps there is a missing case in the productions of "e" to yield "r"?  Otherwise, how can $\exists$ occur under a conjunction (as shown in Section 4.B)?  This is very irksome, because I cannot determine exactly what is expressible in the language.  
\begin{quote}
Please find our answer  to this question in our response to the meta review. Actually, (existential and universal) quantifiers are top level constructs and do not need to appear in the scope of other constructs. All our example test requirements satisfy this restriction. This restriction can be relaxed if in the future we find test requirements for DNNs that need nested quantifiers in their subformulas. 

The formula at the beginning of Section 4.B in the previous version of the paper is an oversight by us, and it has been removed in this new version without affecting the correctness of the other parts. Thank you for pointing this out, and we really appreciate your detailed reading of our paper. 
\end{quote}

\end{revPoint}

\begin{revPoint}
Second, because the paper covers so much ground, there is never a complete definition of the optimization problems that are fed to the solver.  Some of the stages, such as those in the oracle checking distance, would seem to have to be nested inside the optimization queries in order for them to generate sensible test cases, and how this embedding is performed is not made clear by the paper.  I do not understand precisely what optimization problem is being fed to the solver, and my earlier issues with the semantic definitions do not give me the confidence I need to ensure that these translations are being performed correctly.
\begin{quote}
%\youcheng{We do not feed $\arg\max_{x} a: e$ into a solver or a symbolic algorithm, and 
%it is estimated by concretely running the tests in $\testsuites$}
%At the high level, the formula $\arg\max_{x} a: e$ provides all the components that need to be fed into a solver (or a symbolic algorithm). More specifically, $a$ is the optimisation objective, $e$ represents the optimisation constraint, and $x$ is a symbolic representation of a solution. 

The distance can be encoded as a constraint, whose details are provided in Equation (6) of the paper for the Chebyshev distance. 
The Linear Programming (LP) model used each time that encodes an activation pattern is as in 
\eqref{eq:lp-v} and \eqref{eq:lp-dir1}. 
"
Subsequently, the symbolic analysis for finding a new input $t'$ from a pair $(t, r')$ of 
input and requirement is equivalent to finding a new activation pattern. Note that,
to make sure that the obtained test case is meaningful, in the LP model an objective
is added to minimize the distance between $t$ and $t'$."

The oracle checking, however, is not part of the concolic testing. The concolic testing is to generate a set of test cases. This set of test cases are then checked against the oracle to see if they are spurious  or not. The checking is done explicitly since the number of test cases is finite and the checking of a test case againt the oracle can be done in constant time. 

%[xiaowei: how is this related to the question? ] 


\end{quote}

\end{revPoint}

\begin{revPoint}
 In Section 7, I do not understand precisely how the tests t are chosen: are *all* test images run against *all* requirements? 
\begin{quote}
The idea of the selection of pair $(t,r)$ is explained at the beginning of Section 7. We do not run symbolic execution on all pairs, but instead use heuristics to find the most promising pair to proceed. This follows the idea of normal concolic testing. 
That is, the heuristic chooses $t$ by evaluating tests in $\mathcal{T}$ against these requirements that have not been satisfied.


%[xiaowei: ?] 
%The $t$ is chosen by running tests in $\mathcal{T}$ against these requirements that have not been satisfied.
\end{quote}

\end{revPoint}




\begin{revPoint}
Third, because of lack of space, several important experimental details are missing.  Some of these are included in the appendix, but this will not be included in the final published paper.  I do not know how much computational time is required by the approach and whether it can scale to industrial-sized problems, rather than benchmark models.
\begin{quote}
Details of the experiment results are added (please see our response to the meta review).
The experiment setup can be found online now \url{https://github.com/TrustAI/DeepConcolic}. 
\end{quote}

\end{revPoint}

\begin{revPoint}
Minor comments
\begin{quote}
  fixed
\end{quote}
\end{revPoint}


\subsection*{Review \#519B}
\begin{revPoint}
There are four different coverage-based DNN testing methods (DeepXplore, DeepTest, DeepCover, DeepGuage) apart from DeepConcolic, but the authors only compare their results with DeepXplore. Why not to compare all of them? 
\begin{quote}
First, DeepTest and DeepGuage do not release their code, so we are not able to compare with them. We note that DeepTest is mainly based on DeepXplore and DeepGauge is mainly based on FGSM adversarial example generation algorithm, an algorithm taken by DeepXplore as their backbone. For these reasons, we believe it is appropriate to compare with DeepXplore.  

Second, DeepCover (and DeepGauge) considers mainly  a set of new test criteria, while this paper introduces a test case generation approach.

%the main contributions of DeepCover and DeepGuage are the test criteria they propose.
\end{quote}
\end{revPoint}

\begin{revPoint}
In Table 2, DeepConcolic has more than 10\% difference in neuron coverage between $L_{\infty}$  norm and $L_0$  norm for CIFAR-10, but only less than 1\% for MNIST. Does this indicate that DeepConcolic's distance metric is sensitive to dataset, which confutes the statement that "DeepConcolic is generic"? Also, there is no explanation why the distance metric for DeepConcolic is $L_{\infty}$  norm and $L_0$  norm while DeepXplore uses $L_1$  norm. 

When mentioning about the choice of distance metric in the beginning of Section V, it is said that the metric can be a norm based metric like L0, L2, $L_{\infty}$, but then later, in Table 1, the distance metrics are only L0 and $L_{\infty}$. The authors need to explain clearer about those choices. 
\begin{quote}

The DeepConcolic method, as an approach, is generic, since it is applicable to all test requirements that can be expressed with the QLAR logic, when provided with heuristic functions. The expressiveness of the logic in specifying requirements has been exemplified in the paper (Section 5). This is different from other approaches which design dedicated test case generation algorithms for a given (class of) test requirements. 

It is not surprising that a testing approach, such as DeepConcolic, generates test suites of different statistics when working on two programs. The generated test suite is dependent on both the test case generation algorithm and the program itself. 

The experimental results you noticed suggest that, when considering the neuron coverage metric, the CIFAR10 network is more vulnerable to $L_0$ attacks than $L_\infty$ attacks, while this is not the case for the MNIST network.  


"Until now, there is no conclusion on the best distance metric. DeepConcolic 
can be parameterised with a desired norm distance metric $\distance{\cdot}{}$".
$L_{\infty}$ is the most often used. Others like
$L_0$, $L_1$ and $L_2$ are also used in some works. DeepConcolic currently supports $L_{\infty}$
and $L_0$.

\end{quote}
\end{revPoint}


\subsection*{Review \#519C}

\begin{revPoint}
One of the contributions claimed is the use of QLAR to express a set of safety
properties. However, the authors don't make a clear case as to how this new
formalism helps with testing or helps gain insight into the DNN testing
problem. 

\begin{quote}
The key of the QLAR logic is summarized in the following statement: 
"The benefit of a coherent logic framework is
that it not only provides a general way of expressing requirements
(Sections~\ref{sec:concreteRequirement} and \ref{sec:quantification}), but
also enables the resolution of a class of problems with a small set of algorithms
(Section~\ref{sec:symbolic})."

\end{quote}

\end{revPoint}

\begin{revPoint}
Benchmark selection. The authors seem to select one of the smallest benchmarks
   from the DeepXplore work (MNIST) plus another very similar image classification
   benchmark. No mention is made why the other data sets that were
   used to evaluate the prior work are not included in this evaluation.
   In order to claim an improvement over prior work, DeepConcolic needs to
   be evaluated on the same benchmarks as the prior work, listed in table 1
   of the DeepXplore paper. If it is not possible to run DeepConcolic on any
   of these benchmarks, this needs to be explained in the paper.


\begin{quote}
%[xiaowei: not happy with this answer. ] 
%We explicitly state it in the paper this time:
%"Unfortunately, the current DeepConcolic implementation does not support other DNN models
%used in DeepXplore."
The selection of MNIST and CIFAR10 as our benchmark datasets is because they are the status quo for the study of the safety or robustness of DNNs. Our approaches are able to work with larger, state-of-the-art networks, for example in [21] we document the global optimisation approach (briefly introduced in Section 8.2) and its applications to networks trained on ImageNet dataset, including VGG16, VGG19, ResNet, etc. We haven't excised the limit of the linear programming approach on large networks because it is white-box and 
needs a detailed encoding of various hidden layers. Right now, we can encode fully-connected layers, convolutional layers, max pooling layers, and ReLU activation function. Nevertheless, because the underlying computational problem for linear programming is in polynomial time, it is reasonable to believe that the approach can scale well to work with larger networks.  

In the paper, we have made it clear that the comparison with DeepXplore is on MNIST and CIFAR10. Your suggestion on comparing with all the networks studied in the DeepXplore paper is reasonable, and we will keep this in our agenda and distribute the results on the tool's webpage and a future journal version of this paper. As suggested by the other reviewer, the paper has already been ``extraordinarily ambitious''. 
\end{quote}

\end{revPoint}

\begin{revPoint}
%Benchmark selection
%
Experiment repetition for random processes: As soon as there is randomness
   in an experiment it needs to be repeated multiple times and the mean as
   well as the variance should be reported. Obvious randomness in the
   presented evaluation comes from the selection of the image which is said to
   have been random. The experiments should be run with 100-1000 different images
   as starting points to make sure that the good results do not stem from a
   particularly lucky pick of the image input.
\begin{quote}
Added now (please see our response to the meta review).

All coverage results are collected by running the
testing repeatedly at least 10 times.
The full coverage report, including the average coverage and standard derivation, is
given in Figure~\ref{fig:coverage}. The experiment results in Table \ref{tab:NC+DeepConcolic+DeepXplore} and 
\ref{tab:cover-results} have been also updated. 
\end{quote}

\end{revPoint}

\begin{revPoint}
%Benchmark selection
%
   Experiment duration missing: It is customary in software testing to clearly
   indicate how long the testing tool was run for. This is important for
   comparison to other techniques as well as to give the readers an indication
   of how much compute resources and how much time it will take to achieve
   a certain coverage. The run time of all experiments needs to be included
   in the evaluation section.
\begin{quote}
Added now (please see our response to the meta review).

When testing a DNN, if the DeepConcolic testing does not finish
within 12 hours, it is forced to terminate.
%DeepXplore is much faster and terminates in seconds.
Actually, both our approach and DeepXplore are for off-line testing, which is  usually more tolerable on run-time. 
\end{quote}

\end{revPoint}

\begin{revPoint}
In VII.A.2: it is not clear how $c_k$ is calculated
\begin{quote}
Given that the neuron activation values at different layers of a DNN are often of different magnitudes,
$c_k$ is added as a layer-wise constant to normalise activation values at different layers into a comparable level.
Actually, like many machine learning algorithms, $c_k$ is a hyper-parameter of the heuristic, i.e., it is specific to the network the algorithm is working on. In the paper we have provided a way to calculate it:  
"It is estimated by sampling a large enough input dataset".
\end{quote}

\end{revPoint}

\begin{revPoint}
It is not clear what the constraints on the "next input" $t'$ that results
  from the $symbolic\_analysis$ are. This should be clarified.
  \begin{quote}
  To find the new input $t'$, a new activation pattern is first created (Section 8.1.1, 8.1.2 and 8.1.3),
  based on the selected $t$ and $r$.
  Subsequently, this new activation pattern is encoded by the LP constraints using \eqref{eq:lp-v}
  and \eqref{eq:lp-dir1}.
  
  "Note that, to make sure that the obtained test case is meaningful, in the LP model an objective
  is added to minimize the distance between $t$ and $t'$. Thus, the use of LP requires that a distance metric
  be linear, e.g., $L_{\infty}$-norm."
  \end{quote}
\end{revPoint}


\begin{revPoint}
The use of the term "Validity" in Definition 11 is very confusing as it
  normally refers to the question whether a test input is actually a feasible
  input, whereas you are using it to refer to the fact that the test input
  should be close to an existing one.
 \begin{quote}
 Thanks for pointing this out. We have renamed the term "validity" as "soundness" to
 avoid confusion.
\end{quote}
\end{revPoint}



\begin{revPoint}
  it is unclear how "adversarialness" is measured, maybe you can explain
  more about how you compare on this property.
\begin{quote}
The adversarial example is checked using the Robustness Oracle (Definition \ref{def:oracle2}). 
Intuitively, \emph{adversarial examples} are 
"test cases that have different classification labels when close to each other with respect to a distance metric".
%Given a test case $t$, when using the LP model to find a new input $t'$, to make sure that the two
%are close enough, an objective is added to minimize the distance between $t$ and $t'$.
\end{quote}
\end{revPoint}

\subsection*{Review \#519D}

\begin{revPoint}
Four test criteria are used in conjunction. Whereas three of them resemble more traditional notions of coverage, Lipschitz continuity seems to be very specific for DNNs and, at least to me, it is totally new. I would have appreciated some more intuition as to how and why this property makes sense as a test criterion. Can Lipschitz continuity be seen as a robustness metric? If so, can using it as a test criterion be seen as combining functional/structural and non-functional test goals?
\begin{quote}
The Lipschitz continuity of a network has been identified as an important property of a neural network. In the paper, we provide several recent related works (from both verification community and machine learning community) on relating Lipschitz continuity to the robustness of DNNs. Intuitively, with smaller  Lipschitz constant, the network's decision making is less sensitive (and potentially more robust) to the change (or perturbation) of the input. It is therefore  reasonable to use Lipschitz as a test criterion. Please refer to \cite{WWRHK2018,RHK2018} for the details about how to associate the Lipschitz continuity with robustness. 



We agree that Lipschitz testing is  non-functional, since it affects the the way a network operates but usually not directly the behaviour of a network. 
\end{quote}
\end{revPoint}


\begin{revPoint}
There is no formulation of research questions
\begin{quote}
    Section 11 is for experimental results. All the formalisations have been provided in earlier sections. We appreciate the reviewer's comments, and believe it can be more helpful if this comment can be a little more specific. 
    %We are not entirely sure what the reviewer means.
    %Our concolic method is applied to for coverage based testing given criteria including the Neuron Cover, SS Cover and Neuron Boundary Cover. Experiment results show that it achieves high coverage and a significant amount of adversarial examples are detected.
\end{quote}
\end{revPoint}

\begin{revPoint}
Only two datasets were used and their selection is not justified. There is no discussion on the expected external validity of the results presented in the evaluation.
\begin{quote}
    The selection of MNIST and CIFAR10 as our benchmark datasets is because they are the status quo for the study of the safety or robustness of DNNs. Our approaches are able to work with larger, state-of-the-art networks, for example in [21] we document the global optimisation approach (briefly introduced in Section 8.2) and its applications to networks trained on ImageNet dataset, including VGG16, VGG19, ResNet, etc. We haven't excised the limit of the linear programming approach on large networks because it is white-box and 
needs a detailed encoding of various hidden layers. Right now, we can encode fully-connected layers, convolutional layers, max pooling layers, and ReLU activation function. Nevertheless, because the underlying computational problem for linear programming is in polynomial time, it is reasonable to believe that the approach can scale well to work with larger networks.  

    
    %We are not entirely sure what "the expected external validity" means.
\end{quote}
\end{revPoint}

\begin{revPoint}
Random inputs were used to fire the executions of the tool, but there is no account for this randomness in the form of repeated executions.

The discussion notes that the approach generates adversarial examples that "resemble human perception". Since the experiments reported are only for one randomly chosen input, this observation might just be anecdotal.
\begin{quote}
    All results reported in the paper of this new version are collected by running the testing repeatedly for 10 times. We notice that the results do not have significant change from the previous results. 
\end{quote}
\end{revPoint}

\begin{revPoint}
The results section mentions that the different criteria complement each other, but could the authors provide some more insights this cooperation? Is there no scenario in which they might conflict with each other instead? Would a multi-objective search be worth exploring in the future?

\begin{quote}
Thank you for raising this insightful comment. The statement on the complementarity between criteria is not yet rigorously defined in the paper. It comes from our intuitive observations on the experimental results. 
It will be an interesting next step to formalise, and study empirically, the relationship between criteria regarding their effectiveness in guiding the test case generation. The multi-objective search sounds like a good idea. 
Besides, given the same network, the number of adversarial
 examples found under the NC can be quite different when the distance metric is changed. This suggests that, when testing DNNs, one may need to consider multiple distance metrics instead of a single metric. 
 


% This work proposes a concolic testing method that can be conveniently applied to different test criteria.
% Regarding the cooperation between different test criteria, it needs further exploration and is out 
% of the scope of this paper.
% Still, we observed some interesting results. For example, 
 
 
\end{quote}
\end{revPoint}


\begin{revPoint}
There is no discussion about performance in the evaluation section. To have a feeling about this I downloaded and executed the tool (example in README file). It has been about two hours and the tool is still choosing tests at layer 0. The paper could improve if the practical applicability of the approach for ML practitioners was discussed.
\begin{quote}
    We now specify a threshold of 12 hours for each DeepConcolic run.
    When testing a DNN, if the DeepConcolic testing does not finish within 12 hours, it is forced to terminate.
    
    Note that following Algorithm \ref{algo:testing}, the heuristic will pick up the "most promising requirement" each
    time. That means that there is no deterministic order between layers or neurons to test.
\end{quote}
\end{revPoint}

\begin{revPoint}
Minor comments
\begin{quote}
  fixed
\end{quote}
\end{revPoint}

